Causal GNNs: A GNN-Driven Instrumental Variable Approach for Causal Inference in Networks

As network data applications continue to expand, causal inference within networks has garnered increasing attention. However, hidden confounders complicate the estimation of causal effects. Most methods rely on the strong ignorability assumption, which presumes the absence of hidden confounders-an assumption that is both difficult to validate and often unrealistic in practice. To address this issue, we propose CgNN, a novel approach that leverages network structure as instrumental variables (IVs), combined with graph neural networks (GNNs) and attention mechanisms, to mitigate hidden confounder bias and improve causal effect estimation. By utilizing network structure as IVs, we reduce confounder bias while preserving the correlation with treatment. Our integration of attention mechanisms enhances robustness and improves the identification of important nodes. Validated on two real-world datasets, our results demonstrate that CgNN effectively mitigates hidden confounder bias and offers a robust GNN-driven IV framework for causal inference in complex network data.

==> bib.tex <==
@inproceedings{ma2021deconfounding,
  title={Deconfounding with networked observational data in a dynamic environment},
  author={Ma, Jing and Guo, Ruocheng and Chen, Chen and Zhang, Aidong and Li, Jundong},
  booktitle={Proceedings of the 14th ACM International Conference on Web Search and Data Mining},
  pages={166--174},
  year={2021}
}

@inproceedings{guo2021ignite,
  title={Ignite: A minimax game toward learning individual treatment effects from networked observational data},
  author={Guo, Ruocheng and Li, Jundong and Li, Yichuan and Candan, K Sel{\c{c}}uk and Raglin, Adrienne and Liu, Huan},
  booktitle={Proceedings of the Twenty-Ninth International Conference on International Joint Conferences on Artificial Intelligence},
  pages={4534--4540},
  year={2021}
}

@article{veitch2019using,
  title={Using embeddings to correct for unobserved confounding in networks},
  author={Veitch, Victor and Wang, Yixin and Blei, David},
  journal={Advances in Neural Information Processing Systems},
  volume={32},
  year={2019}
}

@inproceedings{ma2023look,
  title={A Look into Causal Effects under Entangled Treatment in Graphs: Investigating the Impact of Contact on MRSA Infection},
  author={Ma, Jing and Chen, Chen and Vullikanti, Anil and Mishra, Ritwick and Madden, Gregory and Borrajo, Daniel and Li, Jundong},
  booktitle={Proceedings of the 29th ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  pages={4584--4594},
  year={2023}
}

@article{rothman2005causation,
  title={Causation and causal inference in epidemiology},
  author={Rothman, Kenneth J and Greenland, Sander},
  journal={American journal of public health},
  volume={95},
  number={S1},
  pages={S144--S150},
  year={2005},
  publisher={American Public Health Association}
}

@article{varian2016causal,
  title={Causal inference in economics and marketing},
  author={Varian, Hal R},
  journal={Proceedings of the National Academy of Sciences},
  volume={113},
  number={27},
  pages={7310--7315},
  year={2016},
  publisher={National Acad Sciences}
}

@article{yazdani2015causal,
  title={Causal inference in the age of decision medicine},
  author={Yazdani, Afsaneh and Boerwinkle, Eric},
  journal={Journal of data mining in genomics \& proteomics},
  volume={6},
  number={1},
  year={2015},
  publisher={NIH Public Access}
}

@article{vanderweele2008causal,
  title={Causal directed acyclic graphs and the direction of unmeasured confounding bias},
  author={VanderWeele, Tyler J and Hern{\'a}n, Miguel A and Robins, James M},
  journal={Epidemiology},
  volume={19},
  number={5},
  pages={720--728},
  year={2008},
  publisher={LWW}
}

@book{pearl2009causality,
  title={Causality},
  author={Pearl, Judea},
  year={2009},
  publisher={Cambridge university press}
}

@inproceedings{zhang2021treatment,
  title={Treatment effect estimation with disentangled latent factors},
  author={Zhang, Weijia and Liu, Lin and Li, Jiuyong},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={12},
  pages={10923--10930},
  year={2021}
}

@inproceedings{jiang2023cf,
  title={Cf-gode: Continuous-time causal inference for multi-agent dynamical systems},
  author={Jiang, Song and Huang, Zijie and Luo, Xiao and Sun, Yizhou},
  booktitle={Proceedings of the 29th ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  pages={997--1009},
  year={2023}
}

@article{forastiere2021identification,
  title={Identification and estimation of treatment and interference effects in observational studies on networks},
  author={Forastiere, Laura and Airoldi, Edoardo M and Mealli, Fabrizia},
  journal={Journal of the American Statistical Association},
  volume={116},
  number={534},
  pages={901--918},
  year={2021},
  publisher={Taylor \& Francis}
}

@inproceedings{cheng2024instrumental,
  title={Instrumental Variable Estimation for Causal Inference in Longitudinal Data with Time-Dependent Latent Confounders},
  author={Cheng, Debo and Xu, Ziqi and Li, Jiuyong and Liu, Lin and Liu, Jixue and Gao, Wentao and Le, Thuc Duy},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={38},
  number={10},
  pages={11480--11488},
  year={2024}
}

@article{angrist1995two,
  title={Two-stage least squares estimation of average causal effects in models with variable treatment intensity},
  author={Angrist, Joshua D and Imbens, Guido W},
  journal={Journal of the American statistical Association},
  volume={90},
  number={430},
  pages={431--442},
  year={1995},
  publisher={Taylor \& Francis}
}

@article{schwartz2012extending,
  title={Extending the sufficient component cause model to describe the Stable Unit Treatment Value Assumption (SUTVA)},
  author={Schwartz, Sharon and Gatto, Nicolle M and Campbell, Ulka B},
  journal={Epidemiologic Perspectives \& Innovations},
  volume={9},
  number={1},
  pages={1--11},
  year={2012},
  publisher={Springer}
}
